Synchronization of Deterministic Visibly Push-Down Automata

We generalize the concept of synchronizing words for finite automata, which map all states of the automata to the same state, to deterministic visibly push-down automata. Here, a synchronizing word w does not only map all states to the same state but also fulfills some conditions on the stack content of each run after reading w. We consider three types of these stack constraints: after reading w, the stack (1) is empty in each run, (2) contains the same sequence of stack symbols in each run, or (3) contains an arbitrary sequence which is independent of the other runs. We show that in contrast to general deterministic push-down automata, it is decidable for deterministic visibly push-down automata whether there exists a synchronizing word with each of these stack constraints, i.e., the problems are in EXPTIME. Under the constraint (1) the problem is even in P. For the sub-classes of deterministic very visibly push-down automata the problem is in P for all three types of constraints. We further study variants of the synchronization problem where the number of turns in the stack height behavior caused by a synchronizing word is restricted, as well as the problem of synchronizing a variant of a sequential transducer, which shows some visibly behavior, by a word that synchronizes the states and produces the same output on all runs.

==> DVPDA-arb-construction.tex <==
\begin{figure}
	\scalebox{0.845}{
	\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm,semithick,state/.style={circle, draw, minimum size=.9cm}]
	
		\draw[fill=gray!20,draw=white] (-1,-4.8) rectangle (12, -3.2);
		\node at (3, -4.5) {$A$};
		
		\draw[fill=gray!40,draw=gray!20] (8,-4) ellipse (3.3cm and .6cm);
		\node at (5.5, -4) {$S$};
	
		\node[state] (1'') {$p''$};
		\node[state] (1') [below of=1''] {$p'$};
		\node[state] (1) [below of=1'] {$p$};
		
		\node[state] (2'') [right of=1''] {$q''$};
		\node[state] (2') [below of=2''] {$q'$};
		\node[state] (2) [below of=2'] {$q$};
		\node [right of=2] {$\dots$};
		\node [right of=2'] {$\dots$};
		\node [right of=2''] {$\dots$};
		
		\node[state] (3'') at (6.5, 0) {$r''$};
		\node[state] (3') [below of=3''] {$r'$};
		\node[state] (3) [below of=3'] {$r$};
		
		\node[state] (4'') [right of=3''] {$s''$};
		\node[state] (4') [below of=4''] {$s'$};
		\node[state] (4) [below of=4'] {$s$};
		\node (S) [right of=4] {$\dots$};
		\node [right of=4'] {$\dots$};
		\node (S'') [right of=4''] {$\dots$};
		
		\node[state] (fin) at (12.5, -2) {$q_{\text{fin}}$};
		\node[state] (stall) [above of=fin]{$q_{\text{stall}}$};
		
	
		
		\path
		(1'') edge [bend left=10] node [pos=0.35] {$a, \push(p)$} (1')
		(1') edge node [pos=0.35]{$a, \push(p)$} (1)
		(1) edge [loop below] node {$a, \push(p)$} (1)
		(1') edge [bend left=10] node {$b, \pop(p)$} (1'')
		(1) edge [bend left=30] node [pos=0.1]{$b, \pop(p)$} (1'')
		(1'') edge [loop above] node {$b, \pop(p)$} (1'')
		%		
		(2'') edge [bend left=10] node {$a, \push(q)$} (2')
		(2') edge node {$a, \push(q)$} (2)
		(2) edge [loop below] node {$a, \push(q)$} (2)
		(2') edge [bend left=10] node [pos=0.35]{$b, \pop(q)$} (2'')
		(2) edge [bend left=30] node [pos=0.1]{$b, \pop(q)$} (2'')
		(2'') edge [loop above] node {$b, \pop(q)$} (2'')
		%
		%
		(3'') edge [bend left=10] node [pos=0.35] {$a, \push(r)$} (3')
		(3') edge  node [pos=0.35]{$a, \push(r)$} (3)
		(3) edge [loop below] node {$a, \push(r)$} (3)
		(3') edge [bend left=10] node {$b, \pop(r)$} (3'')
		(3) edge [bend right=10] node [pos=0.75, above] {$b, \pop(Q)$} (fin)
		(3'') edge [loop above] node {$b, \pop(r)$} (3'')
		%		
		(4'') edge [bend left=10] node {$a, \push(s)$} (4')
		(4') edge  node {$a, \push(s)$} (4)
		(4) edge [loop below] node {$a, \push(s)$} (4)
		(4') edge [bend left=10] node [pos=0.35]{$b, \pop(s)$} (4'')
		(4) edge [bend right=10] node [pos=0.75,below]{$b, \pop(Q)$} (fin)
		(4'') edge [loop above] node {$b, \pop(s)$} (4'')
		%
		(1'') edge [loop left] node [pos=0.3] {$\Sigma_{\text{int}}$} (1'')
		(1') edge [loop left] node [pos=0.3] {$\Sigma_{\text{int}}$} (1')
		(3'') edge [loop left] node [pos=0.3] {$\Sigma_{\text{int}}$} (3'')
		(3') edge [loop left] node [pos=0.3] {$\Sigma_{\text{int}}$} (3')
		(2'') edge [loop right] node [pos=0.7] {$\Sigma_{\text{int}}$} (2'')
		(2') edge [loop right] node [pos=0.7] {$\Sigma_{\text{int}}$} (2')
		(4'') edge [loop right] node [pos=0.7] {$\Sigma_{\text{int}}$} (4'')
		(4') edge [loop right] node [pos=0.7] {$\Sigma_{\text{int}}$} (4')
		%
		(S) edge [bend right=10] node [pos = 0.3, right] {$b, \pop(Q)$}(fin)
		(fin) edge [bend right, color=red] node [left,pos=0.2] {$b, \pop(Q)$} (12, -1)
		(stall) edge [bend right,color=red] node [left, pos=0.2] {$b, \pop(Q)$} (12, 1)
		(fin) edge [bend left=10] node[above] {$b, \pop(\bot)$} (4'')
		(stall) edge [bend right=20] node [above,pos=0.7] {$b, \pop(\bot)$} (4'')
		%
		(fin) edge [loop right] node {$a, \push(F)$} (fin)
		(stall) edge [loop right] node {$a, \push(F)$} (stall)
		(stall) edge [bend left=10] node {$b, \pop(F)$} (fin)
		(fin) edge [bend left=10] node[pos=0.7] {$b, \pop(F)$} (stall)
		;
	\end{tikzpicture}
}
\caption{Illustration of the DVPDA $M$ in the proof of Theorem~\ref{thm:DVPA-Arb-PSPACE}. In a transition $\push(q)$ means that the stack symbol $q$ is pushed on top of the stack with this transition. Similarly, $\pop(q)$ means that the stack symbol $q$ is popped from the stack with this transition. The transitions drawn in red lead to the annotated state $q''$ if the letter $q$ is popped from the stack. For reasons of clarity and comprehensibility, the following transitions are \emph{not} drawn: For $q \in Q, q'\in Q', q''\in Q''$ $\delta'(\{q, q', q''\}, b, p)$ for $q \neq p$; 
$\delta'(\{q_{\text{fin}}, q_{\text{stall}}\}, b, Q)$;
$\delta'(Q \cup Q' \cup Q'', b, \{\bot, F\})$;
$\delta'(Q, \Sigma_{\text{int}})$.
}
\label{fig:DVPDA-Arb}
\end{figure}
